Equivariant Similarity for Vision-Language Foundation Models

This study explores the concept of equivariance in vision-language foundation models (VLMs), focusing specifically on the multimodal similarity function that is not only the major training objective but also the core delivery to support downstream tasks. Unlike the existing image-text similarity objective which only categorizes matched pairs as similar and unmatched pairs as dissimilar, equivariance also requires similarity to vary faithfully according to the semantic changes. This allows VLMs to generalize better to nuanced and unseen multimodal compositions. However, modeling equivariance is challenging as the ground truth of semantic change is difficult to collect. For example, given an image-text pair about a dog, it is unclear to what extent the similarity changes when the pixel is changed from dog to cat? To this end, we propose EqSim, a regularization loss that can be efficiently calculated from any two matched training pairs and easily pluggable into existing image-text retrieval fine-tuning. Meanwhile, to further diagnose the equivariance of VLMs, we present a new challenging benchmark EqBen. Compared to the existing evaluation sets, EqBen is the first to focus on "visual-minimal change". Extensive experiments show the lack of equivariance in current VLMs and validate the effectiveness of EqSim. Code is available at https://github.com/Wangt-CN/EqBen.

==> supp_tables/supp_kubric.tex <==
\begin{table*}[t]
\tablestyle{5pt}{1.5} 
\begin{tabular}{cccccc}
\shline
 & Template & object & verb & location & subject \\ \hline
 \rule{0pt}{30pt}
\multirow{2}{*}{Location} & \multirow{2}{1in}{The $\langle$\textit{object}$\rangle$ $\langle$\textit{verb}$\rangle$ $\langle$\textit{location}$\rangle$ the $\langle$\textit{subject}$\rangle$} & \multirow{6}{2in}{green turtle toy, white animal dog toy, black power pressure cooker, great white shark model, white ramekin porcelain, pink damask bath towel, white porcelain teapot, grey elephant toy, bald eagle toy, brown bull, blue gloves, brown hat, white gaming mouse, black keyboard, black boot, white gift box with red straps, red scissors, vintage metal alarm clock, black frypan, stainless steel milk frother, red coffee mug, purple doll house wooden sofa, black sneaker, white canvas shoe, black laptop, black and red gameboy, blue and black backpack, red high heel, stainless steel toaster, white drug bottle, fabric basket, school bus toy, black and yellow hammer, green doll house wooden refrigerator} & \multirow{4}{1in}{is, is located, is placed} & \multirow{4}{*}{} & \multirow{6}{*}{} \\
 &  &  &  &  &  \\ \cline{1-2}
\multirow{2}{*}{Attribute} & \multirow{2}{*}{} &  &  &  &  \\
 &  &  &  &  &  \\ \cline{1-2}
\multirow{2}{*}{Counting} & \multirow{2}{*}{} &  &  &  &  \\
 &  &  &  &  &  \\ \hline
\end{tabular}
\end{table*}

==> tables/benchmark_table1.tex <==
\begin{table*}[t]
\centering

\tablestyle{3pt}{1.0} 
\begin{tabular}{clccccccccccccl}
\toprule[1.5pt]
&\multicolumn{1}{l}{\multirow{2}{*}{Method}} & \multicolumn{3}{c}{\textsc{Eq-YouCook2}} & \multicolumn{3}{c}{\textsc{Eq-GEBC}} & \multicolumn{3}{c}{\textsc{Eq-AG}} & \multicolumn{3}{c}{Winoground~\cite{thrush2022winoground}} & \multicolumn{1}{c}{\multirow{2}{*}{AVG}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
\multicolumn{1}{c}{} &   & Text & Image & Group & Text & Image & Group & Text & Image & Group & Text & Image & Group & \multicolumn{1}{c}{} \\ \midrule
&LXMERT &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
&CLIP (RN-50)~\cite{radford2021learning} & 47.72 & 47.99 & 34.05 & 10.80 & 18.03 & 3.97 & 14.52 & 10.44 & 3.50 & 25.50 & 11.00 & 8.50  &12.51  \\
&CLIP (ViT-B/32)~\cite{radford2021learning} & 49.48 & 51.10 & 36.50 & 12.57 & 20.12 & 4.47 & 13.91 & 8.72 & 3.32 &30.75  &10.50  &8.00  & 13.07 \\
&FLAVA~\cite{singh2022flava} & 51.66 & 54.78 & 39.68 &12.24  &16.81  &5.07  & 6.59 & 13.47 & 2.15 &32.25  &20.50  &14.25  &14.85  \\
&ViLT~\cite{kim2021vilt} & 44.61 & 46.69 & 31.74 & 14.72 & 16.70 & 5.62 & 15.37 & 9.89 & 3.45 &39.25  &15.75  &11.99  &13.20  \\
&ALBEF~\cite{li2021align} & 57.01 & 58.04 & 44.90 & 13.56 & 19.63 & 5.89 & 11.28 & 15.17 & 3.93 &32.49  &16.50  &12.75  &16.86  \\
&BLIP~\cite{li2022blip} & 59.22 & 58.36 & 46.31 &  15.87 & 19.79 & 7.27 & 19.76 & 13.87 & 6.31 &37.25  &19.49  &14.75  &18.66  \\ \cmidrule(lr){2-15}
&METER~\cite{dou2021empirical} & 52.18 & 49.42 & 36.81 & 20.95 & 18.19 & 6.95 & 28.70 & 15.80 & 7.88 &39.25  &15.75  &11.99  &15.91  \\
&METER-F30K~\cite{dou2021empirical} & 52.68 & 48.31 & 36.52 & 18.08 & 19.85 & 7.33 & 29.50 & 16.30 & 8.12 &39.25  &15.75  &11.99  &16.68  \\
&METER-F30K + \algname &\cellcolor{mygray}\textbf{54.12}  &\cellcolor{mygray}\textbf{53.12}  &\cellcolor{mygray}\textbf{40.29} &\cellcolor{mygray}\textbf{24.20}  &\cellcolor{mygray}\textbf{26.02}  &\cellcolor{mygray}\textbf{11.69} &\cellcolor{mygray}\underline{28.85}  &\cellcolor{mygray}\textbf{20.09}  &\cellcolor{mygray}\textbf{10.76} &\cellcolor{mygray}\textbf{44.99}  &\cellcolor{mygray}\textbf{22.75}  &\cellcolor{mygray}\textbf{18.75}  &\cellcolor{mygray}\textbf{20.37}  \\ \cmidrule(lr){2-15}
&FIBER~\cite{dou2022coarse} & 52.04 & 50.84 & 38.32 & \textbf{25.19} & 22.66 & \textbf{11.08} & \textbf{32.49} & \textbf{24.05} & \textbf{13.70} & 46.25 &25.75  &22.24  &21.34  \\
&FIBER-F30K~\cite{dou2022coarse} & 57.70 & 56.46 & 44.33 & 18.24 & 21.33 & 8.54 & 26.99 & 18.69 & 9.24 &51.24	&26.49  &23.00  & 21.27 \\
\multirow{-12}{*}{\rotatebox{90}{End-to-End}}  &FIBER-F30K + \algname &\cellcolor{mygray}\textbf{58.26}  &\cellcolor{mygray}\textbf{57.10}  &\cellcolor{mygray}\textbf{45.10} &\cellcolor{mygray}\underline{21.55} &\cellcolor{mygray}\textbf{26.07} &\cellcolor{mygray}\underline{10.58} &\cellcolor{mygray}\underline{29.93}  &\cellcolor{mygray}\underline{23.42}  &\cellcolor{mygray}\underline{12.64}  &\cellcolor{mygray}\textbf{51.49}  & \cellcolor{mygray}\textbf{31.49} &\cellcolor{mygray}\textbf{27.50}  &\cellcolor{mygray}\textbf{23.95} \\ \bottomrule[1.5pt]  
\end{tabular}
% }
\caption{Results on three sub-datasets of our proposed \benchname built with natural videos (\textsc{Eq-YouCook2},\textsc{-GEBC},\textsc{-AG}). Additionally, we report results on  text-minimal change benchmark Wingoground~\cite{thrush2022winoground}. ``-F30K'' denotes further fine-tuning on Flickr30K dataset. Rows highlighted in gray are results with our proposed method \algname. Numbers in bold, underline respectively represent the best results and the inferior results compared to pretraining but better than fine-tuning. \linjie{Why do we need underline to highlight these results?} Please check Appendix for the full results due to the space limitation.}
\label{tab:natural}
\end{table*}

==> tables/diagnosis_on_kubric.tex <==
\begin{table*}[t]
\centering
% \captionsetup{font=footnotesize,labelfont=footnotesize,skip=2pt}
% \setlength\extrarowheight{1pt}
\tablestyle{4pt}{1.0} 
\resizebox{\linewidth}{!}{
\begin{tabular}{clccccccccccccl}
\toprule[1.5pt]
&\multicolumn{1}{l}{\multirow{2}{*}{Method}} & \multicolumn{3}{c}{\textsc{Eq-Kubric-Loc.}} & \multicolumn{3}{c}{\textsc{Eq-Kubric-Cnt.}} & \multicolumn{3}{c}{\textsc{Eq-Kubric-Attr.}} & \multicolumn{3}{c}{\textsc{Eq-SD}}  & \multicolumn{1}{c}{\multirow{2}{*}{AVG}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
\multicolumn{1}{c}{} &   & Text & Image & Group & Text & Image & Group & Text & Image & Group & Text & Image & Group & \multicolumn{1}{c}{} \\ \midrule
&LXMERT &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
&CLIP (RN-50)~\cite{radford2021learning} & 7.05 & 6.60 & 1.25 & 18.15 & 15.70 & 5.20 & 38.80 & 43.50 & 22.80 & 90.09 & 85.92 & 79.11 & 27.09  \\
&CLIP (ViT-B/32)~\cite{radford2021learning} & 5.20 & 3.85 & 0.75 & 17.65 & 16.75 & 5.80 & 38.83 & 43.28 & 22.44 & 89.16 & 86.05 & 78.98 & 26.99 \\
&FLAVA~\cite{singh2022flava}  & 8.70 & 6.10 & 1.00 & 22.60 & 18.85 & 7.35 & 55.35 & 59.60 & 39.35 & 79.64 & 84.47 & 71.18 & 29.72  \\
&ViLT~\cite{kim2021vilt} & 11.40 & 7.75 & 1.95 & 19.55 & 14.55 & 6.19 & 62.74 & 58.70 &45.55 & 80.37 & 79.04 & 68.93 & 30.66  \\
&ALBEF~\cite{li2021align} & 7.40 & 6.40 & 1.25 & 21.65 & 24.15 & 9.49 & 60.55 & 60.00 & 44.99 & 88.96 & 90.41 & 83.07 & 34.70  \\
&BLIP~\cite{li2022blip} & 6.49 & 8.60 & 1.15 & 24.65 & 23.55 & 10.60 & 56.99 & 64.59 & 44.44 & 85.39 & 85.52 & 77.13 & 33.33  \\ \cmidrule(lr){2-15}
&METER~\cite{dou2021empirical} & 18.25 & 8.75 & 3.59 & 34.65 & 27.30 & 15.29 & 79.94 & 69.55 & 62.90 & 89.62 & 84.93 & 79.44 & 40.31  \\
&METER-F30K~\cite{dou2021empirical} & 11.29 & 9.49 & 2.40 & 40.50 & 30.19 & 17.49 & 71.54 & 64.09 & 53.10 & 86.64 & 84.46 & 77.46 & 37.61  \\
&METER-F30K + \algname &\cellcolor{mygray}16.69 &\cellcolor{mygray}\textbf{9.70} &\cellcolor{mygray}\textbf{3.80} &\cellcolor{mygray}\textbf{41.45} &\cellcolor{mygray}\textbf{40.25} &\cellcolor{mygray}\textbf{23.85} &\cellcolor{mygray}72.90 &\cellcolor{mygray}67.29 &\cellcolor{mygray}57.60 &\cellcolor{mygray}88.04 &\cellcolor{mygray}84.07 &\cellcolor{mygray}77.79 &\cellcolor{mygray}\textbf{40.76}  \\ \cmidrule(lr){2-15}
&FIBER~\cite{dou2022coarse} & 31.60 & 19.75 & 11.34 & 31.29 & 38.60 & 19.65 & 80.94 & 78.45 & 69.59 & 86.05 & 88.63 & 79.97 & 45.14  \\
&FIBER-F30K~\cite{dou2022coarse} & 29.15 & 15.54 & 8.95 & 43.65 & 46.05 & 28.49 & 78.14 & 76.59 & 66.54 & 90.48 & 86.64 & 81.29 & 46.32 \\
\multirow{-12}{*}{\rotatebox{90}{End-to-End}}  &FIBER-F30K + \algname &\cellcolor{mygray}\textbf{31.90} &\cellcolor{mygray}16.40 &\cellcolor{mygray}11.05 &\cellcolor{mygray}\textbf{43.79} &\cellcolor{mygray}\textbf{49.79} &\cellcolor{mygray}\textbf{30.90} &\cellcolor{mygray}80.00 &\cellcolor{mygray}\textbf{79.00} &\cellcolor{mygray}\textbf{70.20} &\cellcolor{mygray}\textbf{90.81} &\cellcolor{mygray}85.98 &\cellcolor{mygray}80.70 &\cellcolor{mygray}\textbf{48.21} \\ \bottomrule[1.5pt]  
\end{tabular}}
\caption{Results on two sub-datasets of \benchname built upon synthetic engines (\textsc{Eq-Kubri-Loc.},\textsc{-Kubri-Cnt.},\textsc{-Kubri-Attr.},\textsc{-SD}). ``Loc.'', ``Cnt.'' and ``Attr.'' represent location, counting and attribute, respectively.} 
\label{tab:synthetic}
\end{table*}

==> tables/indomain_table.tex <==




\begin{table}[t]
\centering
% \captionsetup{font=footnotesize,labelfont=footnotesize,skip=2pt}
% \setlength\extrarowheight{1pt}
\tablestyle{3pt}{1.0} 
% \scalebox{0.75}{
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule[1.5pt]
% \multicolumn{1}{l}{Method} & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 \\ \midrule
\multicolumn{1}{l}{\multirow{2}{*}{Method}} & \multicolumn{3}{c}{F30K T2I} & \multicolumn{3}{c}{F30K I2T} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& R1 & R5 & R10 & R1 & R5 & R10 \\ \midrule
METER~\cite{dou2021empirical} & 79.60 & 94.96 & 97.28 & 90.90 & 98.30 & 99.50 \\
METER-F30K~\cite{dou2021empirical} & 82.22 & 96.34 & 98.36 & 94.30 & \textbf{99.60} & \textbf{99.90} \\
METER-F30K + \algname & 82.16 & 94.70 & 96.64 & \textbf{95.30} & \textbf{99.60} & \textbf{99.90} \\ \midrule
FIBER~\cite{dou2022coarse} &  &  &  &  &  &  \\
FIBER-F30K~\cite{dou2022coarse} & 81.44 & 96.72 & 98.48 & 92.90 & 99.50 & \textbf{99.90} \\
FIBER-F30K + \algname & \textbf{83.56} & \textbf{96.78} & 98.28 & \textbf{96.00} & \textbf{99.60} & \textbf{99.90}      
\\ \bottomrule[1.5pt]
\end{tabular}}
\caption{Image-text retrieval results on in-domain Flickr-30K~\cite{plummer2015flickr30k} test set.}
\label{tab:indomain}
\end{table}
